Defining Self-adaptive Systems: A Systematic Literature Review

In the last two decades, the popularity of self-adaptive systems in the field of software and systems engineering has drastically increased. However, despite the extensive work on self-adaptive systems, the literature still lacks a common agreement on the definition of these systems. To this day, the notion of self-adaptive systems is mainly used intuitively without a precise understanding of the terminology. Using terminology only by intuition does not suffice, especially in engineering and science, where a more rigorous definition is necessary. In this paper, we investigate the existing formal definitions of self-adaptive systems and how these systems are characterised across the literature. Additionally, we analyse and summarise the limitations of the existing formal definitions in order to understand why none of the existing formal definitions is used more broadly by the community. To achieve this, we have conducted a systematic literature review in which we have analysed over 1400 papers related to self-adaptive systems. Concretely, from an initial pool of 1493 papers, we have selected 314 relevant papers, which resulted in nine primary studies whose primary objective was to define self-adaptive systems formally. Our systematic review reveals that although there has been an increasing interest in self-adaptive systems over the years, there is a scarcity of efforts to define these systems formally. Finally, as part of this paper, based on the analysed primary studies, we also elicit requirements and set a foundation for a potential (formal) definition in the future that is accepted by the community on a broader range.

==> figures/bubble_chart.tex <==
%% only for this demo
%\begin{filecontents*}{myfig.tikz}
  \begin{tikzpicture}
      %\draw (0,0) circle (2cm);
      %\node at (0,0) {Me};
      \tikzset{help lines/.style={color=black!50}}
      \def\pHeight{0.5\columnwidth}
		\def\pWidth{\columnwidth}
		\def\cat{8}
		\def\foo{5}

  %\draw[->] (-5.5,0) -- (5.5,0) node [below] {$s$};
  \foreach \c in {0,1,...,\cat} {
    \draw[thin,help lines] (\c,0) -- (\c,\foo);
  }
  \foreach \c in {0,1,...,\foo} {
    \draw[thin,help lines] (0, \c) -- (\cat,\c);
  }
  \foreach \l [count=\c from 1] in {{Cat 1}, {Cat 2}, {Cat 3}, {}, {Cat 4}, {Cat 5}, {Cat 6}} {
    \node at (\c, -0.2) {\l};
  }
\tikzstyle{stuff_fill}=[rectangle,fill=white!20]
  
   \foreach \l [count=\c from 1] in {{Cat 1}, {Cat 2}, {Cat 3}, {Cat 4}} {
    \node[stuff_fill] at (4, \c) {\l};
  }
  
  %\draw [thick] (0,\y) -- (-0.2,\y);

  \pgfplotstableread{figures/data/map.dat}\table
\pgfplotstablegetrowsof{\table}
\pgfmathsetmacro{\M}{\pgfplotsretval-1}
\pgfplotstablegetcolsof{\table}
\pgfmathsetmacro{\N}{\pgfplotsretval-1}
  \foreach \row in {0,...,\M}{
          \foreach \col in {0,...,\N}{
                 \pgfplotstablegetelem{\row}{[index]\col}\of\table
                 \ifnum\col=0
                       \xdef\x{\pgfplotsretval}
                 \fi
                 \ifnum\col=1
                       \xdef\y{\pgfplotsretval}
                 \fi
                 \ifnum\col=2
                       \xdef\radius{\pgfplotsretval}
                 \fi
                 }
                 \definecolor{mycolor}{RGB}{\pdfuniformdeviate 256,%
                           \pdfuniformdeviate 256,%
                            \pdfuniformdeviate 256}
                 \fill[blue!30,opacity=0.7] (\x,\y)circle({sqrt(\radius/3.1415)*0.4});
                 
                 \node[] at (\x,\y) {\radius};
}
      
  \end{tikzpicture}
%\end{filecontents*}

